A unified Green's function approach for spectral and thermodynamic properties from algorithmic inversion of dynamical potentials

Dynamical potentials appear in many advanced electronic-structure methods, including self-energies from many-body perturbation theory, dynamical mean-field theory, electronic-transport formulations, and many embedding approaches. Here, we propose a novel treatment for the frequency dependence, introducing an algorithmic inversion method that can be applied to dynamical potentials expanded as sum over poles. This approach allows for an exact solution of Dyson-like equations at all frequencies via a mapping to a matrix diagonalization, and provides simultaneously frequency-dependent (spectral) and frequency-integrated (thermodynamic) properties of the Dyson-inverted propagators. The transformation to a sum over poles is performed introducing $n$-th order generalized Lorentzians as an improved basis set to represent the spectral function of a propagator, and using analytic expressions to recover the sum-over-poles form. Numerical results for the homogeneous electron gas at the $G_0W_0$ level are provided to argue for the accuracy and efficiency of such unified approach.

==> bck/main.tex <==

%========================
\section{Introduction}
\label{Introduction}
%========================
Accurate predictions of angle-resolved photo-emission spectroscopy (ARPES) experiments have been the center of great theoretical effort since the mid '50s~\cite{kohn_ground-state_1960,luttinger_ground-state_1960,lundqvist_single-particle_1967,hedin_effects_1970,reining_gw_2018}. Many-body perturbation theory (MBPT) has been extensively used to predict material spectra for extended systems~\cite{reining_gw_2018}, where ground-state theories are often not reliable~\cite{} (e.g. band-gap problem~\cite{}). The knowledge of the one-particle Green's function (GF) grants access to several spectral quantities, e.g. its imaginary part is related to the outcome of an ARPES experiment~\cite{lundqvist_single-particle_1967}. In addition, the GF allows for the calculation of the thermodynamics of a material. The number of particle in a system as well as its total electronic energy can be determined once the GF is known. Though the ingredient is the same, calculations of spectral and thermodynamic quantities differ by methodology and numerical implementation. Indeed, the analytic structure of the Green's function (being it a collection of poles slightly off the real axis for finite systems or a branch cut in the thermodynamic limit~\cite{farid_gw_1988}) requires ad-hoc techniques and approximations to be sampled and used for either scopes. An a priori choice of  the method has to be made in order to predict accurately either material spectra or thermodynamic quantities, where one goal usually excludes the other~\cite{kutepov_electronic_2016}. 

Calculating the total energy or the self-energy (SE) in the most used random-phase approximation (RPA) to the LWK functional once an initial GF is provided, i.e. solving the Hedin's equations for GW non-self consistently ($G_0W_0$), already poses all these issues. The calculation of thermodynamic quantities is typically done evaluating propagators on the imaginary axis, away from their poles and where frequency integrals are easier to perform~\cite{garcia-gonzalez_self-consistent_2001}, but making spectral predictions (real-axis) more involved. On the contrary, to calculate spectra, once the SE has been determined on the real axis, the Dyson equation is solved approximately on isolated frequencies (e.g. with a quasi-particle approximation), thus no integration of the SF over frequency can be carried over, forbidding the calculation of the thermodynamics of the system. Consequently, accuracy for both spectra and thermodynamics can be achieve either improving on analytic-continuation procedures for better spectra or staying on the real axis and targeting precision for frequency-integrated quantities. Focusing on the latter, we note that similar issues on frequency integration are faced when trying to achieve self consistency in Hedin's cycle. The loss of the analytic structure (poles and residues) after the first step (e.g. after a $G_0W_0$ calculation) forbids the use of standard procedures (e.g. plasmon pole or contour deformation) in order to perform convolutions of the subsequent step.

In a series of papers~\cite{von_barth_self-consistent_1996,holm_self-consistent_1997,holm_fully_1998,holm_total_2000} Von-Barth and coworkers partially target these issues, for the homogeneous electron gas, by modelling the SF in frequency-momentum space using Gaussians with $k$-parametrized centers (quasi-particle energies), broadening (weights), and satellites. They also rewrite all $GW$ integrals in terms of the SF in order to make use of the model of the SF. 

%In addition to this, since most techniques to solve Hedin's equations require position and residue of the poles of the GF (e.g. for calculating the SE, the plasmon pole approximation~\cite{} as well as the contour deformation method~\cite{} requires such information), the loss of the knowledge of the analytic structure of the GF after the first iteration of Hedin's equation (i.e. after a $G_0W_0$ calculation) prevent any other step in the self-consistent cycle, unless the interacting propagator (SE) is approximated with a mean field one~\cite{}.
In this paper we develop a unified approach to address the calculation of accurate thermodynamic quantities of a system together with its spectral function, while keeping the analytic structure of the GF explicit at any step during the calculation, and avoiding modellings of the SF. Frequency dependent propagators are expanded as sum-over-poles (SOP) which allows for the analytic calculation of thermodynamic quantities (using the momenta of the GF), analytic convolutions (using Cauchy residue formula), and the solution of the Dyson equation, a procedure we refer to as the algorithmic inversion. For demonstration purposes, we consider the paradigmatic system of the homogeneous electron gas, for several densities ($r_s$ from $1$ to $10$), treated at the non-self-consistent $G_0W_0$ level.

%\AF{At variance to this work, a full frequency treatment of propagators is provided also by the approach developed in Refs.~\cite{von_barth_self-consistent_1996,holm_self-consistent_1997,holm_fully_1998,holm_total_2000}, in which all convolutions between propagators are converted into integrals involving their spectral function, and real parts are obtained afterwards performing a Hilbert transform. We believe the main difference in the two approaches stems in the generalization to non-homogeneous (real) systems. Indeed, the application of those techniques~\cite{von_barth_self-consistent_1996,holm_self-consistent_1997,holm_fully_1998,holm_total_2000} to non-homogeneous systems is not straight-forward and to our knowledge has never been attempted in the literature. On the contrary, being the SOP propagators a sum of single-pole structures (non-interacting propagators weighted by a residue/amplitude) it should not be difficult to use them for a calculation in a real system. For example, starting from the fact that convolutions as well as momenta of SOP represented propagators require summing single-pole objects, the calculation of the LWK functional can be performed equally (apart from computational time) having a $G_0$ Kohn-Sham like propagator, or a full interacting one, e.g. the output of a $G_0W_0$ cycle. Parallel to this example, the aforementioned algorithmic inversion can serve as a tool to solve the Dyson equation in systems where does not exist a diagonal representation of $G_0$ and the SE at all frequencies (real systems, non-homogeneous) without resorting to any approximation (see future work). } \AFnote{to be updated} \AFnote{part of the above probably goes to the discussion/conclusion sections}.
The paper is organized as follows: in~\ref{} we begin introducing the sum-over-poles approach and then in~\ref{} deepen on the analytic of representing frequency-dependent quantities and in~\ref{} the algorithmic inversion; in~\ref{} we propose a numerical example of~\ref{} and~\ref{}; then in~\ref{} we focus on the specific of the calculation for the HEG; in~\ref{} we present our results for spectra and thermodynamics at a single density ($r_s=4$); in~\ref{} we move to the results for several densities; in~\ref{} we conclude and hint to the future work.

%========================
\section{Method}
\label{Method}
%========================
%
In this Section we design and describe the sum-over-poles (SOP) approach to represent frequency-dependent objects such as propagators and self-energies. 
We also introduce the tightly related concept of $n$-th order Lorentians, as a way to improve the decay properties of the represented spectral functions.

As we detail below, the introduction of SOP provides:
($i$) a full frequency treatment of propagators, including
a Kramers-Kronig compliant representation of real and imaginary parts; 
($ii$) analytic frequency integrals (e.g. convolutions and momenta);
($iii$) an approach (algorithmic inversion) to find the solution of the Dyson equation in SOP representation once the equation kernel (e.g. the self-energy or the irreducible polarizability) is given in SOP form. 
%
In order to make the above approach effective, the SOP representation requires:
($v$) a transformation of a frequency-dependent propagator into SOP (in order to pass from a grid to a SOP representation, while the vice versa is granted by SOP itself);
($vi$) a fast decaying of the represented imaginary parts (to avoid Lorentzian tails).
%(which guarantee converging moments until a certain degree);

%In order to make the above approach effective, the SOP representation requires:
%($v$) a transformation of the imaginary part of frequency-dependent propagators into fast-decaying-basis elements (to avoid fat-tail issues)
%($vi$) the analytic SOP form, once the amplitudes on the basis have been fitted.

Here and throughout this article we will focus on the homogeneous electron gas (HEG) for which, due to symmetry the SE and $G_0$ are diagonal in the plane-wave basis. The generalization of the approach to non-homogeneous systems will be the subject of a future work.

%
\subsection{Frequency representation: sum-over-poles and $n$-th Lorentians}
\label{Frequency representation: sum-over-poles and n-th Lorentians}
%
Recalling the single-pole structure of a free propagator, we write any time-order propagator as sum-over-poles (SOP) (for simplicity of notation we suppress any momentum dependence):
\begin{equation}
    G(\omega)=\sum^N_{i} \frac{A^{\mathrm{(SOP)}}_i}{\omega-z_i}
    \label{eq:SOP}
\end{equation}
with $z_i\in \mathbb{C}$ with $\Im{z_i}\gtrless0$ when $\Re{z_i}\lessgtr \mu$ where $\mu$ is the effective chemical potential of the propagator (for a Green's function in the HEG $\mu=\epsilon^0_f$, for the polarizability or the screened potential $\mu=0$) in order to have the correct analytical structure for a TO propagator. The SOP basis is complete (point i) when $\Im{z_i}\to0$ and the number of poles goes to infinity. Indeed, a SOP representation can be thought (at lowest order, see below) as the time-ordered Hilbert transform (TOHT) of a Lorentzian basis
\begin{equation}
    \Im{G(\omega)}=\sum^{N^{(\mathrm{Lor})}}_i A^{(\mathrm{Lor})}_i \frac{\delta_i}{(\omega-\epsilon_i)^2+\delta_i^2}
    \label{eq:lor_basis}
\end{equation}
with $\delta_i\gtrless0$ when $\epsilon_i\lessgtr \mu$ and $A^{(\mathrm{Lor})}_i\ge0$, which for $\delta_i\to0$ is a delta basis for functions that decrease faster than $O(\omega)$. Thus (point ii), to get $G(\omega)$ is sufficient to perform the TOHT analytically:
\begin{eqnarray}
    G(\omega)&=&\frac{1}{\pi}\int_{\mathcal{C}} \frac{\abs{\Im{G(\omega')}}}{\omega-\omega'}d\omega'
    \nonumber \\
    &=& \sum^{N^{(\mathrm{Lor})}}_i A^{(\mathrm{Lor})}_i \int_{\mathcal{C}}\frac{1}{\omega-\omega'}\frac{\abs{\delta_i}}{(\omega'-\epsilon_i)^2+\delta_i^2}d\omega' 
    \nonumber \\
    &=&\sum^N_{i} \frac{A^{\mathrm{(SOP)}}_i}{\omega-z_i}
    \label{eq:TOHT_lor_basis}
\end{eqnarray}
with $N^{(\mathrm{Lor})}=N$ $A^{\mathrm{(SOP)}}_i=A^{(\mathrm{Lor})}_i$ and $z_i=\epsilon_i+i\delta_i$, and where $\mathcal{C}$ is a TO contour which is shifted above the negative-real axis and below the positive-real axis~\cite{holm_self-consistent_1997} with the care that such shift is smaller than all $\delta_i$ and goes to zero after the integral is computed.\\
Without losing point i) and ii), it is possible to generalize eqs~\eqref{eq:lor_basis} and~\eqref{eq:TOHT_lor_basis} to a basis of (here defined) $n$-th order Lorentzians which guarantee fast-decay basis functions (point iii),
\begin{equation}
    \Im{G(\omega)}=\sum^{N^{(n\mathrm{Lor})}}_i A^{(n\mathrm{Lor})}_i \frac{(\delta_i)^{2n-1}}{(\omega-\epsilon_i)^{2n}+(\delta_i)^{2n}},
    \label{eq:nlor_basis}
\end{equation}
for which the SOP representation can be found by doing the TOHT:
\begin{equation}
    \begin{split}
    G(\omega)&=\frac{1}{\pi}\int_{\mathcal{C}} \frac{\abs{\Im{G(\omega')}}}{\omega-\omega'}d\omega' \\
    &=\sum^{N^{(n\mathrm{Lor})}}_i A^{(n\mathrm{Lor})}_i \int_{\mathcal{C}}\frac{1}{\omega-\omega'}\frac{\abs{\delta_i}^{2n-1}}{(\omega'-\epsilon_i)^{2n}+(\delta_i)^{2n}}d\omega
    \label{eq:TOHT_nlor_basis}
    \end{split}
\end{equation}
where each element of the sum in the rhs can be obtained by expanding $\frac{\abs{\delta_i}^{2n-1}}{(\omega-\epsilon_i)^{2n}+(\delta_i)^{2n}}=\prod_{k=0}^{2n-1} \frac{\abs{\delta_i}^{2n-1}}{z-\omega_0-e^{i\frac{\pi}{2n}\left(1+2k\right)}\delta_i}$, and get the TOHT of a single $n$-th order Lorentzian as
\begin{equation}
     A^{(n\mathrm{Lor})}_i\int_{\mathcal{C}}\frac{1}{\omega-\omega'}\frac{\abs{\delta_i}^{2n-1}}{(\omega'-\epsilon_i)^{2n}+(\delta_i)^{2n}}d\omega' =\sum^n_{m} \frac{ A^{\mathrm{(SOP)}}_{i,m}}{\omega-\zeta_{i,m}}
    \label{eq:amp_nlor_basis}
\end{equation}
with $A^{\mathrm{(SOP)}}_{i,m}=2iA^{(n\mathrm{Lor})}_i\prod_{l=0,\ l\neq m}^{2n-1} e^{-i\frac{\pi}{2n}} \left(e^{i\frac{m\pi}{2}}-e^{i\frac{l\pi}{2}}\right)^{-1}$ and $\zeta_{i,m}=\epsilon_i+e^{i\frac{\pi}{2n}\left(1+2m\right)}\delta_i$. We note that $n$-th Lorentzian assure absolute convergence of their moments up to the $2n-1$ order (see below) and their overlap is necessarily smaller, assuring a more orthogonal and easy to treat basis than smaller-degree slower-decaying Lorentzians.\\ 
From a propagator defined on grid we get it's SOP representation (point iv) by performing a non-negative-least-square (NNLS) fit~\cite{lawson_solving_1995,virtanen_scipy_2020} on the amplitudes using an $n$-th order Lorentzian basis fed with the imaginary part of the propagator, and then use eqs.~\eqref{eq:TOHT_nlor_basis} and~\eqref{eq:amp_nlor_basis} to have the SOP representation.\\
The Cauchy integral formula can be used to compute convolution between SOP's (point v):
\begin{equation}
\begin{split}
    &\frac{1}{2\pi i}\int_{-\infty}^{+\infty}G(\omega+\omega')\Tilde{G}(\omega')d\omega'\\
    &=\frac{1}{2\pi i}
    \sum_{i,j} A^{\mathrm{(SOP)}}_i \Tilde{A}^{\mathrm{(SOP)}}_j \int_{-\infty}^{+\infty}
    \frac{1}{\omega+\omega'-z_i}\frac{1}{\omega'-\Tilde{z_j}}d\omega'\\
    &= \sum_{\substack{i,j \\ \Im{z_i>0} \\ \Im{\Tilde{z}_j<0}}} \frac{A^{\mathrm{(SOP)}}_i \Tilde{A}^{\mathrm{(SOP)}}_j}{z_i-\Tilde{z_j}-\omega}+
    \sum_{\substack{i,j \\ \Im{z_i<0} \\ \Im{\Tilde{z}_j>0}}} \frac{A^{\mathrm{(SOP)}}_i \Tilde{A}^{\mathrm{(SOP)}}_j}{\omega+\Tilde{z_j}-z_i}
\end{split}
\label{eq:convolutionSOP}
\end{equation}
closing the contour above. And any integral of the kind (point vi)
\begin{equation}
    E^{\mathrm{R}}[\omega^n]=\frac{1}{2\pi i}\lim_{\eta\to0^+}\int_{-\infty}^{+\infty} e^{i\eta\omega}\omega^n G(\omega)=\sum_{\substack{i \\ \Im{z_i>0}}} A^{\mathrm{SOP}}_i z^{n}_i
    \label{eq:regularizedMomenta}
\end{equation}
which we will refer to as the $n$-th regularize moment of $G$ in SOP. If we use an $n$-th order Lorentzian basis to represent $G(\omega)$ in SOP, the $2(n-1)$ regularize moment will coincide with the occupied moment of its spectral function (done here with a single $n$-th Lorentzian for simplicity):
\begin{equation}
\begin{split}
    E^{\mathrm{R}}[\omega^{2(n-1)}]=\frac{1}{2\pi i}\lim_{\eta\to0^+}\int_{-\infty}^{+\infty} e^{i\eta\omega}\omega^{2(n-1)} G(\omega)\\
    =\frac{1}{\pi}\frac{1}{2\pi i}\lim_{\eta\to0^+}\int_{-\infty}^{+\infty} \int_{\mathcal{C}}\frac{e^{i\eta\omega}\omega^{2(n-1)}}{\omega-\omega'}\\\frac{\abs{\delta}^{2n-1}}{(\omega'-\epsilon)^{2n}+(\delta)^{2n}}d\omega' \ d\omega\\
    =\frac{1}{\pi}\frac{1}{2\pi i}\int_{\mathcal{C}}\lim_{\eta\to0^+}\int_{-\infty}^{+\infty} \frac{e^{i\eta\omega}\omega^{2(n-1)}}{\omega-\omega'}\\\frac{\abs{\delta}^{2n-1}}{(\omega'-\epsilon)^{2n}+(\delta)^{2n}}d\omega \ d\omega'\\
    =\frac{1}{\pi}\int_{-\infty}^{\mu} (\omega')^{2(n-1)} \frac{\abs{\delta}^{2n-1}}{(\omega'-\epsilon)^{2n}+(\delta)^{2n}} d\omega'=\\\int_{-\infty}^{\mu} \omega^{2(n-1)} A(\omega)  d\omega'
    =E^{\mathrm{occ}}[\omega^{2(n-1)}]
    \end{split}
    \label{eq:occupiedMomenta}
\end{equation}
where $A(\omega)=\frac{1}{\pi}\abs{\Im{G(\omega)}}$ is the spectral function of $G$ and we stress that we exchanged the integrals in $d\omega$ and $d\omega'$ thanks to the fast decay of the $n$-th Lorentzian and the calculation of the $2(n-1)$ moment (the same derivation would hold for lower degree moments).
%
\subsection{Dyson inversion on SOP}
\label{Dyson inversion on SOP}
As anticipated in the introduction, within the SOP approach the solution of the Dyson equation is remapped into a diagonalization (point vii), a procedure we call algorithmic inversion (AI). Throughout this article we will concentrate in the special case of the HEG, the treatment of the non-homogeneous case will be the subject of a later publication. Suppressing the $k$ momentum index for simplicity, let us suppose to have the SOP representation of the SE $\Sigma(\omega)=\sum_{i=1}^{N}\frac{\Gamma_i}{\omega-\sigma_i}$ and $G_0=\frac{1}{\omega-\epsilon_0}$ be a non-interacting SOP. By expanding the SOP representation of SE and $G_0$, the Dyson equation can be rewritten as
\begin{equation}
\begin{split}
     G(\omega)=\left[G_0^{-1}(\omega)-\Sigma(\omega)\right]^{-1}=\frac{1}{\omega-\epsilon_0-\Sigma(\omega)}\\=
     \frac{(\omega-\sigma_1)\cdots(\omega-\sigma_N)}{T_N(\omega)},
     \label{eq:Dyson_G}
\end{split}
\end{equation}
in which the $N+1$ roots of the polynomial
\begin{equation}
\begin{split}
     T_N(\omega)=&(\omega-\epsilon_0)(\omega-\sigma_1)\cdots(\omega-\sigma_N)
     \\&-\Gamma_1(\omega-\sigma_2)\cdots(\omega-\sigma_N)-\dots
     \\&-\Gamma_N(\omega-\sigma_1)\cdots(\omega-\sigma_{N-1}),
\end{split}
\end{equation}
are the poles of the Green's function, indeed this is the case when we have $N$ poles in the SE. The roots of $T_N$ are the eigenvalues of the algorithmic inversion $\left(N+1\right)\times \left(N+1\right)$ matrix
\begin{equation}
    \mathrm{AIM}=\begin{pmatrix}
        \epsilon_0 & \sqrt{\Gamma_1} & \dots & \sqrt{\Gamma_N}\\
        \sqrt{\Gamma_1} & \sigma_1 & 0 & 0 \\
        \vdots & 0 & \ddots & 0\\
        \sqrt{\Gamma_N} & 0 & \dots & \sigma_N
\end{pmatrix}.
\end{equation}
We prove this statement by observing that the characteristic polynomial of the AIM is $(-1)^{N-1}T_N$, where the sign is just there for the equality and will not matter for the roots. We proceed by induction. Since the $N=1$ case is trivial we move to the $N$-th case. Via Laplace onto the last line, the characteristic polynomial of the $N$-th case can be reduced to 
\begin{equation}
\begin{split}
    p_\mathrm{AIM}(\omega)&=\begin{vmatrix}
        \epsilon_0-\omega & \sqrt{\Gamma_1} & \dots & \sqrt{\Gamma_N}\\
        \sqrt{\Gamma_1} & \sigma_1-\omega & 0 & 0 \\
        \vdots & 0 & \ddots & 0\\
        \sqrt{\Gamma_N} & 0 & \dots & \sigma_N-\omega
\end{vmatrix}\\
&=(\sigma_N-\omega) (-1)^{N-2} T_{N-1}(\omega)+
\\ & +(-1)^{N} \sqrt{\Gamma_N}
\begin{vmatrix}
        \sqrt{\Gamma_1} & \dots & \sqrt{\Gamma_{N-1}} &  \sqrt{\Gamma_N}\\
        \sigma_1-\omega & 0 & 0& 0 \\
        0 & \ddots & 0 & 0\\
        0 & \dots & \sigma_{N-1}-\omega & 0
\end{vmatrix}
\end{split}
\end{equation}
where we have used the induction hypotheses in the first addend of the rhs. Again using Laplace on the last column for the second addend
\begin{equation}
\begin{split}
    p_\mathrm{AIM}(\omega)&=(-1)^{N-2}(\sigma_N-\omega) T_{N-1}(\omega) \\ &- \Gamma_N(\sigma_1-\omega)\cdots(\sigma_{N-1}-\omega)=(-1)^{N-1}T_N(\omega)
\end{split}
\end{equation}
concludes the proof.\\
Calling $\epsilon_i$ the (eigenvalues of the AIM) poles of $G$ we calculate the residues equating
\begin{equation}
    G(\omega)=\sum_{i=1}^{N+1}\frac{A_i}{\omega-\epsilon_i}=
    \frac{(\omega-\sigma_1)\cdots(\omega-\sigma_N)}
    {(\omega-\epsilon_1)\cdots(\omega-\epsilon_{N+1})}
\end{equation}
and using the Heaviside cover-up method~\cite{thomas_calculus_1988} (same residue for the two functions):
\begin{equation}
    A_i=\frac{(\epsilon_i-\sigma_1)\cdots(\epsilon_i-\sigma_N)}
    {(\epsilon_i-\epsilon_1)\cdots(\epsilon_i-\epsilon_{i-1})(\epsilon_i-\epsilon_{i+1})\cdots(\epsilon_i-\epsilon_{N+1})}.
    \label{eq:amps_AI}
\end{equation}
Thus we have proven that with $\Sigma$ in SOP the SOP of $G$ is found throughout 
the AI procedure (diagonalization of AIM plus Eq.~\eqref{eq:amps_AI}).\\
In the paper we will use not only the AI for the SE but also the one for the polarizability $P$ in order to get the SOP of the correlated part of the screened potential $W_\mathrm{corr}(\omega)=W(\omega)-v_c=v_c\left(\frac{1}{1-v_c P(\omega)}-1\right)$, where $v_c$ is the Coulomb potential (recalling that we are suppressing the momentum dependence for simplicity). To invert 
\begin{equation}
    \frac{1}{1-v_c P(\omega)}=\frac{\omega}{\omega}\frac{1}{1-v_c P(\omega)}=\frac{\omega}{\omega-\omega v_c P(\omega)}
    \label{eq:Dyson_w}
\end{equation}
we can use
$\omega v_c P(\omega)=\sum_i \omega\frac{v_c{S}_i}{\omega-g_i}=v_c S_1+\dots+v_c S_N+\sum_i \frac{v_c g_i{S}_i}{\omega-g_i}:=c_0-C(\omega)$ and thus have $\frac{1}{1-v_c P(\omega)}=\frac{\omega}{\omega-c_0-C(\omega)}$, for which the AIM can be used to find the poles of $W_\mathrm{corr}$. Amplitudes of $W_\mathrm{corr}$ are easily found using again the equality against residues (note that by doing $\frac{\omega}{\omega}$ we have inserted a pole in $0$ which we need to discard as the eigenvalue of the AIM since will have zero residue thanks to the numerator $\omega$ of the rhs of eq.~\eqref{eq:Dyson_w}, consequently $P$ and $W_\mathrm{corr}$ will have the same number of poles).

%========================
\section{Numerical verification}
\label{Numerical verification}
%========================
%
In this section we exemplify numerically some properties of the SOP.\\
As test case for points i) to iv) we consider a most different function from the $n$-th Lorentzian basis, the Faddeeva~\cite{virtanen_scipy_2020} function, i.e. the retarded (just for this test case we work with retarded propagators) HT of a Gaussian, and want to represent it both in a Lorentzian basis and $2$ nd order Lorentzian basis. We choose to feed the NNLS fitting algorithm with $10$ points (of the imaginary part) and $9$ $1$ st and $2$ nd order Lorentzians centered on the midpoint between two adjacent points and broadened with the width of the interval (in order to ensure an exhaustive cover of the domain). We use then eqs.~\eqref{eq:TOHT_nlor_basis} and~\eqref{eq:amp_nlor_basis} to get the SOP representation of the fitted Lorentzians and realize it on a finer grid. The scope is to see how much the fitted and then represented SOPs differ from the true one, especially away from the fitting points. As anticipated in the previous section, the upper panel of Fig.~\ref{fig:fadeevaVsLorWithMeans} shows that with a faster-decay Lorentzian a more accurate result is obtained both for real (left) and imaginary (right) parts. In the lower panel we compare the momentum of the Faddeeva function with those obtained from eq.~\eqref{eq:regularizedMomenta} and eq~\eqref{eq:occupiedMomenta}. Since absolute convergence for the first and second moment is not ensured for $1$ st order Lorentzian (i.e. eq~\eqref{eq:occupiedMomenta} does not hold), $E^{\mathrm{R}}[\omega^{n>1}]$ has to be calculated with~\eqref{eq:regularizedMomenta} and in general will be complex. In order to obtain a meaningful result we take the real part and consider the imaginary as an error that must be controlled with a convergence procedure $\delta_i\to0$ approaching the delta basis limit. Not surprisingly faster-decay Lorentzians perform better.\\
As a test for the AI, we consider the example case of a TO SE with $8$-th poles and a free propagator $G_0$ with one occupied pole. We show the SE grid realization in the upper panel of Fig.~\ref{fig:AI_example}. In the lower panel a comparison is drawn between the $G$ obtained with the Dyson inversion on grid against the inversion on poles (AI), i.e. use the AI ti obtain $G$ on SOP and then realize it on grid. The result is at the precision of the calculated eigenvalue of the AIM since the amplitude calculation of eq~\eqref{eq:amps_AI} should be very precise and should not contribute to the error significantly. 

%========================
\section{Details of the calculations}
\label{sec:Details of the calculations}
%========================
%
We will test the SOP approach in a real calculation. We choose to target an homogeneous system (HEG) in a one shot $G_0W_0$ calculation in order to produce a working example of the SOP approach in MBPT. Since we will calculate propagators on the real-axis we can safely assume that our results are accurate for the spectral frequency-dependent properties (we will trust the comparison with the existent literature), but check the accuracy and stability of the frequency-integrated ground-state quantities (occupation number, total energy et cetera) which can be obtained directly from the SOP of the spectral quantities found in the procedure. We stress that usually~\cite{rojas_space-time_1995,rieger_gw_1999,garcia-gonzalez_self-consistent_2001} thermodynamic properties are targeted thanks to additional calculations of propagators on the imaginary axis, while in this work we use their SOP representation obtained with the calculated on the real-axis.

\subsection{Spectral propagators on the real axis}
\label{Details of the calculations - Spectral propagators on the real axis}
We will solve a one shot-cycle for the spin-unpolarized HEG. The first of the integrals to be computed is
\begin{equation}
\begin{split}
    P(q,\omega)=&\frac{2}{(2\pi)^3}\int d\mathbf{k}
    \\& \left(\frac{1}{2\pi i}\int_{-\infty}^{+\infty} G(\omega+\omega',\abs{\mathbf{k+q}})G(\omega',k)\right)
    \label{eq:polarizabilityInt}
\end{split}
\end{equation}
for the polarizability. We will integrate analytically on frequency applying eq.~\eqref{eq:convolutionSOP}. Then integrate numerically on spherical coordinates by performing the change of variables $x=\abs{\mathbf{k+q}}$ on the azimuthal angle of $\mathbf{k}$, which allows the pre-calculation of the analytical convolution on the two dimensional $(x,k)$ grid, instead of on the three dimensional $(k,q,\theta)$ grid. Exploiting the parity of $P(\omega)$, it is possible to limit the $\mathbf{k}$ integration to the occupied states, since $P(\omega)=P_{\mathrm{occ}}(\omega)-P_{\mathrm{unocc}}(\omega)=P_{\mathrm{occ}}(\omega)+P_{\mathrm{occ}}(-\omega)$~\cite{fetter_quantum_2003}. The numerical integration on the momentum is performed using the trapezoidal rule, which ensures exponential convergence for decaying functions.\\
For the self-energy integral
\begin{equation}
\begin{split}
    \Sigma(k,\omega)=&\Sigma_x(k)+\frac{1}{(2\pi)^3}\int d\mathbf{q} \\&\left(\frac{1}{2\pi i}\int_{-\infty}^{+\infty} G(\omega+\omega',\abs{\mathbf{k+q}})W_\mathrm{corr}(\omega',q)\right)
    \label{eq:sigmaIntegral}
\end{split}
\end{equation}
we can still use eq.~\eqref{eq:convolutionSOP} since we will suppose to have the SOP of $W$ obtained with the fit on $P(\omega)$ and then the AI. We again perform the $x=\abs{\mathbf{k+q}}$ change of variable which allows for fewer convolutions, and use trapezoidal weights as in eq.~\eqref{eq:polarizabilityInt} for the momentum integration.\\
In Fig.~\ref{fig:flow_charts_spectral} we show the flow chart from a GF to a SE of the (FORTRAN90) \texttt{heg\_sgm.x} program, implementing the SOP approach for the HEG in the GW approximation (the code is published on Github at~\cite{}).

\subsection{Frequency integrated quantities and thermodynamics} \label{Details of the calculations - Frequency integrated quantities and thermodynamics}
As said previously, the SOP approach allows for accurate and converged calculations of spectral as well as thermodynamic quantities. The algorithmic inversion here plays a central role assuring consistency in all sum-rules respected by a propagator and its Dyson inversion, e.g. between the SE and the GF. Thus using the AI and eq.~\eqref{eq:regularizedMomenta}, the knowledge of the SOP of the SE grants the analytic calculation if the SF occupied (spectral) moments, which are necessary for the thermodynamics. To calculate e.g. the total energy we perform a NNLS fitting on $\Gamma=\frac{1}{\pi}\abs{\Im{\Sigma}}$ (since the SOP form of the SE will not be known as it comes from eq.~\eqref{eq:sigmaIntegral}) and algorithmically invert it to get the SF. We note that performing a fit on $\Gamma$ is somewhat easier (faster converging in the number of points) than fitting the SF, since $\Gamma$ has only divergences while $A$ has (e.g. for $k\to k_f$) $\frac{1}{\omega}$ behaviours.\\
We calculate the total energy with the Galitski-Migdal (GM) formula~\cite{}
\begin{equation}
\begin{split}
    E&=\int d\mathbf{k}\ \left( \int_{-\infty}^{\mu}A(k,\omega)\omega\ d\omega+
    k^2\int_{-\infty}^{\mu}A(k,\omega)\ d\omega\right)\\
    &=\int d\mathbf{k}\ \bigg( \expval{\epsilon_k}+
    k^2 n_k\bigg),
\end{split}
\label{eq:Galitski-Migdal}
\end{equation}
performing the frequency integral with eq.~\eqref{eq:regularizedMomenta} (regularized moments), allowed by the use of the AI. Indeed, as it can be seen from the imaginary part of the Dyson equation $A=\frac{1}{\pi}\frac{\Im{\Sigma}}{(\omega-\epsilon_0-\Re{\Sigma})+(\Im{\Sigma})^2}$, the SF decays as $\frac{\Im{\Sigma}}{\omega^2}$ and so will do  the SF obtained from the SOP for $G$ from an AI (being it exact). In section~\ref{Results - Frequency integrated quantities and thermodynamics} we study the convergence of the total energy $E$. We then plot the the occupation factor $n_k$~\cite{luttinger_ground-state_1960}, the occupied band $\expval{\epsilon_k}$, and the total-energy-momentum density $e_k$ (rhs of eq.~\eqref{eq:Galitski-Migdal}), from the converge calculation. In Fig.~\ref{fig:flow_charts_total_ene} the flow chart for the calculation of the energy in the~\texttt{heg\_sgm.x} program is shown.

%========================
\section{Results}
\label{Results}
%========================
%
In this section we discuss the results obtained applying the SOP approach to the test case of a $G_0W_0$ calculation for the HEG. We focus on the most studied $r_s=4$ density, giving the results for $r_s$ from one to ten at the end of this section.

\subsection{{\label{Results - Spectral propagators on the real axis}} Spectral propagators on the real axis}
In Fig.~\ref{fig:polarizabilityPlotCalsVsTheory} we compare the calculated (using eq.\eqref{eq:polarizabilityInt}) and SOP represented (fitted to a $2$ nd order Lorentzian with NNLS and then realized on a frequency grid) imaginary-part of polarizability with its analytic expression~\cite{fetter_quantum_2003} (note that this is the only analytic result we can use as a check, everything else we need to evaluate strictly numerically). The $\delta\to0^+$ broadening in $G_0$ used in order to converge the numerical momentum integration, seems not to affect qualitatively the calculation. We stress that this is achieved thanks to an input spectral function of $2$ nd order fast-decaying Lorentzians which are converted into SOP using eq.~\eqref{eq:amp_nlor_basis}, which is an accelerator of convergence for the thermodynamic limit $\delta\to0^+$. From the plot comparison, we can infer qualitatively we are converged in all the numerical procedures, i.e. momentum integration, broadening, and NNLS fitting of the resulting polarizability.\\
We shall look at the SE numerical procedures examining directly the spectral function in Fig.~\ref{fig:spectralFuncG0W0rs4}. This is obtained calculating eq.~\eqref{eq:sigmaIntegral}, representing the SE on SOP with $2$ nd order Lorentzians, Dyson inverting the SE on SOP to get the SOP for $G$ (AI), and then realizing the SOP representation on a frequency grid. Posing the attention on the satellite as well as on the  quasi-particle band, Fig.~\ref{fig:spectralFuncG0W0rs4} compares well with~\cite{pavlyukh_dynamically_2020} (note that at variance with~\cite{virtanen_scipy_2020}, we used a logarithmic scale to represent the intensity of the spectral function in order to highlight its structure). A peculiar feature arises for small momenta where the quasi-particle band broadens while the satellites in the occupied-frequency range ($\omega<\mu$) are more peaked. Vice-versa, the standard picture of a more-peaked quasi-particle band is restored as $k$ approaches $k_f$, which results at $k=k_f$ in the analytical divergence of the quasi-particle band at $\hbar\omega=\mu$, where satellites should be almost of the same weight~\cite{von_barth_self-consistent_1996}. For $k>k_f$ satellites coming from empty states ($\omega>\mu$) become dominant along with the quasi-particle band.

\subsection{Frequency integrated quantities and thermodynamics} \label{Results - Frequency integrated quantities and thermodynamics}
We study convergence and stability of the occupation number $n_k$, the occupied band $\epsilon_k$ and the total energy from eq.~\eqref{eq:Galitski-Migdal} (GM). We use the SF on SOP obtained following section~\ref{Results - Spectral propagators on the real axis}, and eq.~\eqref{eq:regularizedMomenta} to get either $n_k$ or $\epsilon_k$. For a complete convergence study of the total energy, we need to converge: all the border domains to infinity $q^\mathrm{max}$ (maximum of the screen-potential-momentum grid), $\omega^\mathrm{max}_{W}$ (maximum of the screen-potential-frequency grid), $k^\mathrm{max}$ (maximum of the SE-momentum grid), $\omega^\mathrm{max}_{\Sigma}$ (maximum of the SE-frequency grid); the refine parameter $\Delta \to 0^+$ which control all frequency-momentum-grid spacing and Lorentzian broadening $\delta$ following $\Delta = \Delta k_P = 5\Delta x_{P} = \frac{1}{6}\Delta\omega_{W} = \frac{1}{9}\Delta q_{P}  =\frac{1}{25} \Delta\omega_{\Sigma} = \Delta x_{\Sigma} = \frac{1}{3}\Delta k_{\Sigma}=\frac{5}{4}\delta_P=\frac{1}{100}\delta_\Sigma$, which are respectively 
$\Delta k_P$ (momentum-spacing $k$ of eq.~\eqref{eq:polarizabilityInt}), 
$\Delta x_{P}$ (momentum-spacing $x$ of eq.~\eqref{eq:polarizabilityInt}), 
$\Delta\omega_{W}$ (frequency-spacing $\omega$ of eq.~\eqref{eq:polarizabilityInt}),
$\Delta q_{P}$ (momentum-spacing $q$ of eq.~\eqref{eq:polarizabilityInt}),
$\Delta\omega_{\Sigma}$ (frequency-spacing $\omega$ of eq.~\eqref{eq:sigmaIntegral}),
$\Delta x_{\Sigma}$ (momentum-spacing $x$ of eq.~\eqref{eq:sigmaIntegral}),
$\Delta k_{\Sigma}$ (momentum-spacing $k$ of eq.~\eqref{eq:sigmaIntegral}),
$\delta_P$ (broadening $\delta$ of eq.~\eqref{eq:polarizabilityInt}),
$\delta_\Sigma$ (broadening $\delta$ of eq.~\eqref{eq:sigmaIntegral}). Note that we do not need to converge the NNLS fits (for $B$ and $\Gamma$) since as in the example of section~\ref{Numerical verification} we place the $2$ nd order Lorentzians on the midpoint between two adjacent points of the frequency grid with a broadening equal to the interval size (to ensure an exhaustive cover), thus converging the frequency-grid-spacing $\Delta\omega$ converges also the fit. 

In Fig.~\ref{fig:totEnecG0W0rs4} a convergence study in all these parameters is given. The convergence value is $0.0381 \pm 0.0002 \ \mathrm{Ha}$ in agreement with~\cite{garcia-gonzalez_self-consistent_2001} (with a difference of $0.0003$ Ha) in which calculations were done along the imaginary axis. In the left panel of Fig.~\ref{fig:frequencyIntegratedG0W0} we examine $n_k$ (upper part) and $\epsilon_k$ (lower part). The occupation number presents a sharp Luttinger discontinuity, which indicates the broadening used in eq.~\eqref{eq:sigmaIntegral} is negligible. In the right panel of Fig.~\ref{fig:frequencyIntegratedG0W0} we plot the total-energy-momentum-density of the GM formula (rhs of eq~\eqref{eq:Galitski-Migdal}). Due to the presence of the Luttinger discontinuity, this function is sharp and thus difficult to integrate, making it unfavorable to be used to calculate the total energy $E$ with respect to e.g. the RPA-Klein functional, which should be smoother in the momentum.

\subsection{$G_0W_0$ for a broad range of densities in the HEG}
\label{Results - $G_0W_0$ for a broad range of densities in the HEG}
In this section we show the results for $r_s$ from $1$ to $10$ of the HEG in a $G_0W_0$ calculation following the same strategy as for the $r_s=4$ density.
In Fig.~\ref{fig:spectralFuncG0W0severalrs} we show the results for the spectral function obtained with our calculation. In the chosen units (of $\epsilon_f$ for the energy and $k_f$ for the momentum) the spectral function for growing $r_s$ shows an increase in the separation between the quasi-particle band and the satellite occupied-empty bands. Indeed, in these units $r_s$ varies the interaction strength ---see eq.~(3.24) in~\cite{fetter_quantum_2003}--- with the limits of the non-interacting $r_s\to0$ gas and the strongly interacting gas for $r_s\to\infty$. The same limits can be observed for the occupation factor of Fig.~\ref{fig:occFactseveralrs} for the different densities. For $r_s\to0$ the gas approaches the non-interacting limit and the quasi-particle weight drops from $1$ to $0$ for growing $k/k_f$. Whereas for $r_s=10$ the quasi-particle weight (proportional to the jump in $n_k$) is smaller since the weight is shared with the satellites bands, as it can be seen from Fig.~\ref{fig:occFactseveralrs}. In table~\ref{tab:corelation_ene} we report the corresponding total energies at the different densities along with the available (to our knowledge) results in the literature. Since calculations of~\cite{garcia-gonzalez_self-consistent_2001} were done on the imaginary axis, we shall consider those as the most accurate for the comparison. At $rs=1$ we find the maximum discrepancy of $0.0059$ Ha with~\cite{garcia-gonzalez_self-consistent_2001}, where we expect more numerical problem being $n_k$ a steeper function and thus the gas more metallic for smaller $r_s$. We did not investigate further the reason of the discrepancy. Instead, we stress that at variance with~\cite{garcia-gonzalez_self-consistent_2001}, our procedure provides not only accurate frequency-integrated quantities (e.g. the total energy), but also precise spectral properties on the real axis (key quantities for experimental spectroscopy).

In table~\ref{tab:fit_parameters_PZ} we find the values of $\gamma$, $\beta_1$, and $\beta_2$ of the fitting function for the correlation energy of the HEG~\cite{von_barth_self-consistent_1996,ceperley_ground_1980}:
\begin{equation}
    E_\mathrm{corr}(r_s)=\frac{\gamma}{1+\beta_1\sqrt{r_s}+\beta_2 r_s}
    \label{eq:perdew_zunger_fit}
\end{equation}
and the covariance matrix of the fit. We also plot the fitting-function of eq.~\eqref{eq:perdew_zunger_fit} with the parameters of table~\ref{tab:fit_parameters_PZ} in Fig.~\ref{fig:table_tot_ene_complete}.


%========================
\section{Conclusions and future perspectives}
%========================
%
In this paper we develop the (so-called) SOP approach, designed to target the full frequency dependence of propagators in MBPT. Building from the standard $1$-pole structure of non-interacting propagators, we prove it is possible to write any propagators as sum-over-poles (SOP). We generalize SOP forms in order to use not only Lorentzians as spectral functions of propagators (e.g. as in the textbook non-interacting case) but $n$-th order generalized Lorentzians, characterized by a faster decay at infinity, and thus provide better numerical stability (smaller basis overlaps for fitting procedures), improved analytical properties (the first $2n-1$ momenta are assured absolute convergence), and faster convergence to the $\delta\to0^+$ thermodynamic limit. We use the SOP representation of propagators to compute convolutions eq.~\eqref{eq:convolutionSOP} as well as spectral (occupied) momenta eq.~\eqref{eq:occupiedMomenta} (using the Cauchy residue theorem), in order to compute spectral as well as thermodynamic quantities, e.g. the $GW$ self-energy or the total energy with the GM formula. Finally, we prove that within the SOP approach the solution of a Dyson equation is mapped into a diagonalization problem, a procedure we call the algorithmic inversion.\\
To have a working example of the SOP approach, we study the test case of a $G_0W_0$ calculation for the HEG at several densities ($r_s$ from $1$ to $10$). Using SOP, we are able to provide accurate spectra as well as precise frequency-integrated quantities (e.g. occupation number and total energy). For the spectral function, we find very good agreement with~\cite{pavlyukh_dynamically_2020}. Moving to the total energy, we provide an in depth study of the stability and convergence of our results, finding quantitative agreement with~\cite{garcia-gonzalez_self-consistent_2001}, where calculation are done on the imaginary axis.\\
Being the SOP approach designed to treat interacting systems with a frequency dependence, it's application to self-consistent solutions of Hedin's equations (e.g. in the RPA approximation) is straight forward and a further publication is already in preparation.\\
Although in this article we study a homogeneous system (HEG) as test case, the SOP approach is designed to be extended for the treatment of real (non-homogeneous) crystals, granting a full-frequency representation of (interacting) propagators, the flexibility for self-consistent calculations, and allowing the exact solution of a Dyson equation through the algorithmic inversion. All of these topics will be the subject of future work. 




==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> paper_aux_manual.tex <==



==> sec_method_representation_v1.tex <==

%========================
\section{Method: AIM-SOP for dynamical potentials}
\label{sec:method_SOP}
%========================
%
In this Section we introduce the algorithmic-inversion method to treat dynamical (frequency-dependent) potentials. The crucial goal for AIM-SOP is to solve exactly and at all frequencies Dyson-like equations for dynamical potential expressed as sum over poles.
For this purpose we express frequency-dependent propagators and self-energies (or, say, polarizabilities or screened Coulomb interactions) in a SOP form:
\begin{equation}
    G(\omega)=A_0 + \sum^N_{i=1} \frac{A_i}{\omega-z_i},
    \label{eq:SOP}
\end{equation}
where the constant term $A_0$ may be present for self-energies and potentials.
Generally, we consider here having complex residues $A_i$ and poles $z_i=\epsilon_i+i\delta_i$ ($\epsilon_i,\delta_i\in \mathbb{R}$).
In order to provide the correct analytical structure respecting time-ordering, $\delta_i\gtrless0$ when $\epsilon_i\lessgtr \mu$, where $\mu$ is the effective chemical potential of the propagator (for a Green's function  $\mu$ is the Fermi energy of the system, for a polarizability or a screened potential $\mu=0$). 
%As detailed below, the SOP form of Eq.~\eqref{eq:SOP} can also be seen as a Pad\`e approximant, i.e. a ratio of polynomials of degree $N-1$ at the numerator and $N$ at the denominator, opening the way to exploiting Pad\`e-specific algorithms when available.
%and, while we differ somewhat in the way we find the Pad\`e coefficients (poles and residues), a comparison between standard Pad\`e techniques for the interpolation~\cite{Lee1996PRB} and the one developed in this article is drawn in Sec.~\ref{}.}

% In Sec.~\ref{sec:method_representation} and~\ref{sec:method_transform} we focus on the transformation to SOP, with an overview in Sec.~\ref{sec:method_representation} on the connection between a propagator and its spectral function and its representation to SOP using different SOP-compliant basis sets, and in~\ref{sec:method_transform} on the transformation to SOP in practice.
% In Sec.~\ref{sec:method_analytical} we give several useful expressions when dealing with propagators on SOP, such as analytic convolutions and moments. In Sec.~\ref{sec:validation} we give a numerical example of a representation on SOP for a trial grid-defined propagator. 
% Finally, in Sec.~\ref{sec:Dyson_SOP} we present the algorithmic-inversion method for the solution on SOP of the Dyson equation. We give a mathematical proof for the case of a self-energy on SOP, and then we discuss the polarizability inversions. At the end we build with a numerical example as proof-of-concept for the procedure.

%We begin with an overview in Sec.~\ref{sec:method_representation} of the connection between a propagator and its spectral function, first for a continuum and then extending it to treat spectral functions represented on discrete basis sets, as will be used in this work. Then, we consider different basis sets to represent the spectral function and obtain a SOP representation introducing $n$-th order Lorentzians. In Sec.~\ref{sec:method_transform} we provide the numerical procedure to transform a propagator sampled on grid to a SOP representation, and viceversa. In Sec.~\ref{sec:method_analytical} we introduce several useful expressions when dealing with propagators on SOP, such as analytic convolutions and moments, and in Sec.~\ref{sec:validation} we show with a numerical example the representation on SOP for a trial grid-defined propagator. Finally, in Sec.~\ref{sec:Dyson_SOP} we present the algorithmic-inversion method on sum-over-poles for the exact solution on SOP of the Dyson equation. We provide a mathematical proof for the case of a self-energy on SOP, and then we discuss the case of the polarizability inversion, concluding with a numerical example as proof-of-concept for the procedure.

Throughout this work we will use as case of study the homogeneous electron gas (HEG) also in view of to the extensive algorithmic and numerical results in the literature. In the HEG, due to translational symmetry, the two-point operators (including Green's functions, self-energies, polarizabilities) are diagonal on the plane-wave basis, but the AIM-SOP can be generalized to non-homogeneous systems, as will be discussed in future work.


%Besides representation, this approach also allows for a more efficient calculation of the propagators themselves (e.g. by exploiting the analytical properties of the representation) and for an exact solution of Dyson-like equations (see Sec.~\ref{sec:Dyson inversion on SOP}). 
%Last, we also introduce the concept of $n$-th order Lorentians, as a way to improve the decay properties of the spectral functions obtained from the SOP representation.


%More specifically, the introduction of SOP provides:
%($i$) a full frequency treatment of propagators, including
%a Kramers-Kronig compliant representation of real and imaginary parts;
%($ii$) analytic frequency integrals (e.g. convolutions and momenta);
%($iii$) an approach (algorithmic inversion) to find the solution of the Dyson equation in SOP representation once the equation kernel (e.g. the self-energy or the irreducible polarizability) is given in SOP form. 
%
%In order to make the above approach effective, the SOP representation requires:
%($v$) a transformation of a frequency-dependent propagator into SOP (in order to pass from a grid to a SOP representation, while the vice versa is granted by SOP itself);
%($vi$) a fast decaying of the represented imaginary parts (to avoid Lorentzian tails).
%(which guarantee converging moments until a certain degree);

%\AFnote{later as a summary of the first part of the  theory?}

%In order to make the above approach effective, the SOP representation requires:
%($v$) a transformation of the imaginary part of frequency-dependent propagators into fast-decaying-basis elements (to avoid fat-tail issues)
%($vi$) the analytic SOP form, once the amplitudes on the basis have been fitted.


%=============
\subsection{Spectral representations}
%: sum-over-poles and $n$-th Lorentians
\label{sec:method_representation}
%=============
%
Following Ref.~\cite{holm_self-consistent_1997}, we consider the spectral representation of a propagator (here the Green's function for simplicity), where $G$ is expressed in terms of its spectral function $A$,
\begin{eqnarray}
    G(\omega)&=&\int_{\mathcal{C}} \frac{A(\omega')}{\omega-\omega'} \, d\omega'
    \label{eq:TOHT}
\end{eqnarray}
%which allows us to pass from $A$ to $G$ 
by performing a
time-ordered Hilbert transform (TOHT), where $\mathcal{C}$ is a time-ordered contour which is shifted above/below the real axis for $\omega' \lessgtr\mu$, 
%$\mu$ is the effective chemical potential defined above, 
and where the shift is sent to zero after the integral is computed.
% SOLVED
%\AFnote{Qui il contour implica che $A(\omega)$ e' valutata per $\omega$' complesso, cioe' stiamo usando la continuazione analitica di $A$. Vogliamo usare questa notazione cmq ? Quasi preferisco $i0^+ \text{sgn}(\mu-\omega')$ al denominatore.}\TCnote{secondo me visto che Von barth fa così questa scrittura riprende la sua formula quindi e' ok, ma capisco il punto.}
%
Accordingly, the inverse relation to go from $G$ to $A$ is given by:
%
\begin{eqnarray}
  \label{eq:G_to_A}
  A(\omega)&=&\frac{1}{2\pi i}\left[ G(\omega) -G^\dagger(\omega) \right]\,\text{sgn}(\mu-\omega) \\
  &=& \frac{1}{\pi} \text{Im}G(\omega)\,\text{sgn}(\mu-\omega),
  \nonumber
\end{eqnarray}
the last expression being valid for a scalar Green's function, as is the case for the HEG.
%note that this is valid only in a homogeneous system where operators are diagonal and thus the spectral function is real, for a in-depth discussion refer to~\cite{farid_gw_1988,martin_interacting_2016}).
%
Representing the spectral function on a (finite) basis set $\{b_j(\omega)\}$,
\begin{equation}
    A(\omega)=\sum_j a_j b_j(\omega)\, \text{sgn}(\mu-\epsilon_j) = 
    \sum_j a_j 
    \abs{b_j(\omega)},
    \label{eq:A_representation}
\end{equation}
with $b_j(\omega)$ centred on $\epsilon_j$ and positive (negative) for $\epsilon_j\lessgtr\mu$, respectively, and $a_j>0$, we also induce a representation of $G$. This is achieved by introducing a discrete time-ordered Hilbert transform (D-TOHT) as
\begin{eqnarray}
    G(\omega)&=& \sum_{j} a_j \int \frac{\abs{b_j(\omega')}}{\omega-\omega'-i0^+ \ \text{sgn}(\mu-\epsilon_j)} \, d\omega',
    \label{eq:TOHTdiscrete}
\end{eqnarray}
where the sign chosen for $b_j$ in Eq.~\eqref{eq:A_representation} gives by construction the time-ordered analytic structure of the Green's function.
In the case of all $\delta_j\to0$ with the number of $b_j$ becoming infinite (continuum representation limit), Eq.~\eqref{eq:TOHTdiscrete} becomes the standard TOHT of Eq.~\eqref{eq:TOHT} (with $\mathcal{C}$ shifted by $\pm i0^+$). 

%Thus, representing $\text{Im}G(\omega)$ on a basis,
%\begin{equation}
%    \text{Im}G(\omega) = \sum_j a_j b_j(\omega),
%    \label{eq:imG_representation}
%\end{equation}
%with $b_j$ positive/negative-localized functions centred on $\epsilon_j  \lessgtr\mu$ and $a_j>0$, yields a representation for the spectral function via Eq.~\eqref{eq:G_to_A}, with 
%\begin{equation}
%   A(\omega)=\sum_j a_j b_j(\omega) \text{sgn}(\mu-\epsilon_j) = 
%    \sum_j a_j 
%    \abs{b_j(\omega)}\,.
%    \label{eq:A_representation}
%\end{equation}
%Accordingly, it is possible to define the discrete-time-ordered Hilbert transform (D-TOHT) as
%\begin{eqnarray}
%    G(\omega)&=& \sum_{j}\alpha_j \int \frac{\abs{b_j(\omega')}}{\omega-\omega'-i\eta \ \text{sgn}(\epsilon_j)} \, d\omega',
%    \label{eq:TOHTdiscrete}
%\end{eqnarray}
%(for $\eta\to0^+$), where in the case of an infinite basis set Eq.~\eqref{eq:TOHTdiscrete} converges to the standard TOHT of Eq.~\eqref{eq:TOHT} (with $\mathcal{C}$ shifted by $\eta$).

A natural choice is to use a basis of Lorentzian functions centered at different frequencies $\epsilon_j$, according to:
%If we represent the spectral function $A$ using Lorentzian-basis elements $\mathcal{L}_i$, each centred at $\epsilon_i$ and with broadening $\delta_i$ 
%(same convention on the signs as in~\eqref{eq:SOP}),
\begin{equation}
    |b_j(\omega)|=\mathcal{L}_{\delta_j}(\omega-\epsilon_j) = \frac{1}{\pi} \frac{\abs{\delta_j}}{(\omega-\epsilon_j)^2+\delta_j^2},
    \label{eq:1lor_basis}
\end{equation}
%
for which the D-TOHT for the single element is analytical, yielding a pole function $1/(\omega-z_j)$ with $z_j=\epsilon_j+i \delta_j$, with the sign convention for $\delta_j$ defined as discussed above according to time ordering.
%
Thus, choosing $b_j$ as in Eq.~\eqref{eq:1lor_basis} induces a SOP representation for $G$ according to Eq.~\eqref{eq:SOP}, with  
$A_i =a_i \in \mathbb{R}$. Once the SOP representation of $G$ is known, i.e. poles and amplitudes are known, the grid evaluation (inverse of the above) is trivial and amounts to performing the finite sum in Eq.~\eqref{eq:SOP}.
%
%in the space of functions that decrease faster than $O(\omega)$) 
This approach ensures a full-frequency treatment of the propagator (approaching the continuum representation limit where Lorentzians becomes delta functions), while preserving 
an explicit knowledge of the analytical structure and continuation of $G$.
%the possibility to pass from a grid evaluation to a SOP representation, transforming $A(\omega)$ onto a Lorentzian basis, using centers and broadenings of the Lorentians as poles and the coefficients on the basis as residues.
%
%Recalling the analytical properties of time-ordered propagators, we adopt a sum-over-poles (SOP) expression to represent any propagator (including also polarizabilities, self-energies and frequency-dependent potentials) according to:
%
%\begin{equation}
%    G(\omega)=\sum^N_{i} \frac{A^{\mathrm{SOP}}_i}{\omega-z_i}
%    \label{eq:SOP}
%\end{equation}
%(for simplicity of notation we suppress any momentum dependence).
%Here $z_i=\epsilon_i+i\delta_i\in \mathbb{C}$ with $\delta_i\gtrless0$ when $\epsilon_i\lessgtr \mu$ where $\mu$ is the effective chemical potential of the propagator (for a Green's function  $\mu$ is the Fermi energy of the system, for the polarizability or the screened potential $\mu=0$) in order to have the correct analytical structure due to time-ordering. 
%
%\AF{Equation~\eqref{eq:SOP} represents then the propagator $G$ as a meromorphic function with a finite number of poles.} 
%Loosely speaking, the SOP basis becomes complete \AF{in the space XXX} \AFnote{shall we mention something about the space?} (point $i$) when $\Im{z_i}\to0$ and the number of poles goes to infinity. 

%Moreover, since each $1/(\omega-z_i)$ term in Eq.~\eqref{eq:SOP} is the time-ordered Hilbert transform (TOHT, see below for the precise definition), of a Lorentzian function centered at $\epsilon_i$ and with broadening $\delta_i$, the SOP representation also fulfills the TOHT/Kramers-Kronig relations by construction: 
%
%\begin{eqnarray}
    %\frac{1}{\pi}
%    \Im{G(\omega)} &=&
    %\frac{1}{\pi}
%    \sum^{N}_i \text{Re}A^{\mathrm{SOP}}_i \frac{\delta_i}{(\omega-\epsilon_i)^2+\delta_i^2} 
%    \nonumber \\
%    &+& 
%    \sum^{N}_i \text{Im}A^{\mathrm{SOP}}_i \frac{\omega-\epsilon_i}{(\omega-\epsilon_i)^2+\delta_i^2}
%    \label{eq:lor_basis}
%\end{eqnarray}
%
%with $\delta_i\gtrless0$ when $\epsilon_i\lessgtr \mu$ and $A^{\mathrm{Lor}}_i\ge0$, which for $\delta_i\to0$ is a delta basis for functions that decrease faster than $O(\omega)$. 
%Thus (point $ii$), to get $G(\omega)$ is sufficient to perform the TOHT analytically:
%
%with $N^{\mathrm{Lor}}=N$ $A^{\mathrm{SOP}}_i=A^{\mathrm{Lor}}_i$ and $z_i=\epsilon_i+i\delta_i$, and 
%
%In Eq.~\eqref{eq:TOHT_lor_basis}, $\mathcal{C}$ is a time-ordered contour which is shifted above (below) the real axis for $\omega' <\mu$ ($\omega' >\mu$)~\cite{holm_self-consistent_1997} with the care that such shift is smaller than all $\delta_i$ and goes to zero after the integral is computed.
%
%In view of Eqs.~(\ref{eq:SOP}-\ref{eq:lor_basis}), the SOP approach induces also a representation of the spectral function $A(\omega)=\frac{1}{\pi}\text{Im}G(\omega)\,\text{sgn}(\mu-\omega)$ of the propagator $G$, particularly evident in Eq.~\eqref{eq:lor_basis} when $A^{\text{SOP}}_i$ are real, $\delta_i\to0$, and the number of poles goes to infinity.
%(at least for real $A^{\text{SOP}}_i$ coefficients), and an equivalent representation of the $G$ spectral function is induced:

%\subsection{Improving decay properties: N-th order Lorentians}

The main drawback of using Lorentzians to represent $G$ is related to the slowly decaying tails ($1/\omega^2$ for $\omega \to\infty$) induced in the spectral function when using finite broadening values $\delta_j$.
%Focusing on the representation of the spectral function and without losing properties ($i$) and ($ii$), it is possible to pass from a basis of Lorentzians to 
%
In order to improve on this, we introduce here $n$-th order generalized Lorentzians to obtain fast-decay basis functions. These are defined as
%
\begin{eqnarray}
    \abs{b_j(\omega)} = \mathcal{L}_{\delta_j}^n(\omega-\epsilon_j) = 
    \frac{1}{N_n\pi} \frac{\abs{\delta_j}^{2n-1}}{(\omega-\epsilon_j)^{2n}+(\delta_j)^{2n}},
    \label{eq:nlor_basis}
\end{eqnarray}
where 
%$N_n = \frac{1}{n \sin(\frac{\pi}{2n})}$ 
$N_n = \left[n \sin(\frac{\pi}{2n})\right]^{-1}$ 
is the normalization factor (see Appendix~\ref{sec:SOP_nLor}).
%
The D-TOHT of $\mathcal{L}_\delta^n$ remains analytic and still yields a SOP representation for $G$ (see Appendix~\ref{sec:SOP_nLor}):
%(using the residue theorem for the integration):
\begin{equation}
    \label{eq:TOHT_nlor_basis}
%    \frac{1}{N_n\pi }\int_{\mathcal{C}}\frac{d\omega'}{\omega-\omega'-i\eta \ \text{sgn}(\epsilon_j)}\frac{\abs{\delta_j}^{2n-1}}{(\omega'-\epsilon_j)^{2n}+(\delta_j)^{2n}} %\ d\omega' 
%    \\=
    \int_{\mathcal{C}} d\omega'\frac{\mathcal{L}_{\delta_j}^n(\omega'-\epsilon_j)}{\omega-\omega'-i0^+\,  \text{sgn}(\mu-\epsilon_j)} 
       =
    \sum^{n-1}_{m=0} \frac{ \alpha_{m}}{\omega-\zeta_{j,m}},
\end{equation}
%
with residues $\alpha_{m}$ and poles $\zeta_{j,m}$ given by
%
\begin{eqnarray}
\label{eq:TOHT_nlor_basis_res}
\alpha_{m} &=&\frac{1}{i N_n n} e^{i\frac{\pi}{2n}\left(1+2m\right)} \\[5pt]
\zeta_{j,m}&=&\epsilon_j+e^{i\frac{\pi}{2n}\left(1+2m\right)}\delta_j\, .
\label{eq:TOHT_nlor_basis_poles}
\end{eqnarray}

Importantly, $\alpha_{m}$ are complex (and so become the residues $A_i=a_j \alpha_{m}$  in the SOP representation, $i$ being a combined index).
Thus, the spectral function of this SOP has contribution by both the real and the imaginary part of each Lorentzian pole $1/(\omega-\zeta_{j,m})$, resulting in a overall faster decay than each single Lorentzian. Also, it is worth noting that, as for standard Lorentzians, a normalized $n$-th-order-Lorentzian approaches a Dirac delta for $\delta_j\to0^+$.
%owing the fact $\mathcal{L}_{\delta_j}^n(\omega-\epsilon_j)=\frac{1}{N_n\pi\delta_j}\left[1+\left(\frac{\omega-\epsilon_j}{\delta_j}\right)^{2n}\right]^{-1}$. 
Owing to their fast decay and to this last property, using a SOP for $G_0$ in term of $n$-th Lorentzians provides a faster convergence for $\delta\to 0^+$, in comparison with a SOP representation built on ordinary Lorentzians, as will be also shown later. While the use of $n$-th order generalized Lorentzians to represent the spectral function $A(\omega)$ provides a faster decay in the imaginary-part of the propagator, it results in a multiplication of the number of poles in the SOP for $G$ (by the degree of the Lorentzian), and in having complex residues. As it will be shown in Sec.~\ref{sec:method_analytical}, the decay properties are fundamental for evaluating the moments of a SOP representation, assuring absolute convergence up to order $2(n-1)$. Also, the use of faster decay basis elements when representing the spectral function improves on the stability of the representation procedure, reducing the off-diagonal elements of the overlap matrix of the basis (see Sec.~\ref{sec:method_transform}).

Alternatively to $n$-th order Lorentzians, one could consider e.g. using Gaussian functions to represent $A(\omega)$, and consequently $G(\omega)$, as done in Refs.~\cite{von_barth_self-consistent_1996,holm_self-consistent_1997}.
Gaussians also allow for an analytical expression of the D-TOHT, at the price, though, of invoking the Dawson~\cite{Abramowitz1965book} or Faddeeva~\cite{virtanen_scipy_2020} functions to evaluate the real part of the propagator. Because of this, SOP expressions are not available, and basic operations involving propagators (such as those described in Sec.~\ref{sec:method_analytical}) cannot be evaluated analytically and need to be worked out in other ways, e.g. numerically or recasting the expressions in terms of propagator spectral functions~\cite{von_barth_self-consistent_1996}.

%=======
\subsection{Transform to a sum over poles}
%=======
\label{sec:method_transform}
%
Once the SOP representation has been introduced, the next important step is to determine numerically the SOP coefficients $A_i$ in Eq.~\eqref{eq:SOP}, given an evaluation of $G$ on a frequency grid.
According to the discussion of Sec.~\ref{sec:method_representation}, the SOP representation can be seen equivalently as a representation for the Green's function $G$ or for the spectral function $A$.

As a first case, we consider representing $A(\omega)$ according to Eq.~\eqref{eq:A_representation}, and we do it using the basis of $n$th-order generalized Lorentzians introduced in Eq.~\eqref{eq:nlor_basis}.
First, we obtain the coefficients $a_j$ of the representation by performing a non-negative-least-square (NNLS) fit~\cite{lawson_solving_1995,virtanen_scipy_2020}, thus assuring the positivity of all $a_j$. Then, we use Eqs.~(\ref{eq:TOHT_nlor_basis_res}-\ref{eq:TOHT_nlor_basis_poles}) to get the SOP representation for the propagator.
While the position and broadening $(\epsilon_j,\delta_j)$ of the $n$-th order Lorentzians could also be optimized by means of a non-linear NNLS fit, here we consider them centred at $\epsilon_j=\frac{1}{2}\left(\omega_j+\omega_{j-1}\right)$ and broadened with $\delta_j=\abs{\omega_j-\omega_{j-1}}$, and we just linearly optimize $a_j$. Also, for numerical reasons we prefer to work with the bare imaginary part of $G$, i.e. without imposing the sign factor of Eq.~\eqref{eq:G_to_A}, since this function is smoother than the actual spectral function $A(\omega)$ close to the Fermi level.

%Once obtained, the $a_j$ coefficients of Eq.~\eqref{eq:A_representation} will be used to get the $A_i$ residues in Eq.~\eqref{eq:SOP} as discussed after Eqs.~(\ref{eq:TOHT_nlor_basis_res}-\ref{eq:TOHT_nlor_basis_poles}). This step is equivalent to analytically perform the D-TOHT on the represented $A(\omega)$ and therefore generates a propagator $G$ that is time-ordered and Kramers-Kronig compliant.
%
%to get a SOP representation for a time-ordered-propagator evaluated on grid, we first recover the imaginary part and then represent it
%on a $n$-th-order-generalized-Lorentzian basis as given in Eq.~\eqref{eq:nlor_basis}. 
%Since $A(\omega)$ is positive definite for the exact Green's function (as well as for well-constructed approximations~\cite{stefanucci2016prl}, including GW), a property inherited by $a_j$ in the infinite basis set limit (when the $n$th Lorentzians become Dirac delta's), we decide to impose the positiveness of the $a_j$ coefficients. To do so
%In order to have Kramers-Kroenig~\cite{} relationship between the real and the imaginary part of the transformed propagator $G$ on SOP with the correct sign (positive representation coefficients), 
% we perform a non-negative-least-square (NNLS) fit~\cite{lawson_solving_1995,virtanen_scipy_2020} of $A(\omega)$ on the amplitudes $a_j$. %using an $n$-th-order-generalized-Lorentzian basis 
% Frequency sampling points $\omega_j$ of $A$ are chosen to be uniform.
% While the position and broadening $(\epsilon_j,\delta_j)$ of the $n$-th order Lorentzians could also be optimized by means of a non-linear LS fit, here we consider them uniformly distributed -- with $\epsilon_j=\frac{1}{2}\left(\omega_j+\omega_{j-1}\right)$ and  $\delta_j=\abs{\omega_j-\omega_{j-1}}$ -- and we just linearly optimize $a_j$. Also, for numerical reasons we prefer to work with the bare imaginary part of $G$, i.e. without imposing the sign factor of Eq.~\eqref{eq:G_to_A},  this function being smoother than the actual spectral function $A(\omega)$ close to the Fermi level.


Alternatively, one could consider the basis representation induced on $G$ via Eq.~\eqref{eq:SOP} in order to directly obtain the $A_i$ and $z_i$ coefficients (residues and poles). As for $A(\omega)$, this can be achieved by a linear or non-linear LS fit (or interpolation) taking advantage of the knowledge of the whole $G(\omega)$ on a frequency grid (and not just of $A$).
Interestingly, the SOP representation in Eq.~\eqref{eq:SOP} is a special case of a Pad\`e approximant, written as the ratio of polynomials of order $N-1$ and $N$, respectively.
Because of this, one can exploit Pad\`e-specific approaches to determine ($A_i$,$z_i$), such as, for instance, Thiele's recursive scheme~\cite{Lee1996PRB}.
We found that this leads to a very efficient method when few tens of poles are considered, becoming numerically unstable beyond. Moreover, since the residues are not constrained to be real and positive ($A_i$ are actually complex), there is no control over the time-ordered position of the poles, and the procedure is non-trivial to extend to the case of $n$-th order Lorentzians. For the above reasons, in the present work we adopt the first approach, based on the representation of $A(\omega)$.


%=======
\subsection{Analytical expressions}
%=======
\label{sec:method_analytical}
%
Once the SOP representation of a dynamical propagator is available, a number of analytical expressions hold.
For instance, the convolution of propagators, such as those involved in the evaluation of the independent-particle polarizabilities in terms of the Green's functions, can be evaluated using Cauchy's residue theorem:
%
\begin{multline}
    \int_{-\infty}^{+\infty}  \frac{d\omega'}{2\pi i} \,G(\omega+\omega')\Tilde{G}(\omega')d\omega' = \\
    =
    \sum_{i,j} \int_{-\infty}^{+\infty}
    \frac{d\omega'}{2\pi i} \, \frac{A_i}{\omega+\omega'-z_i}\,\frac{\Tilde{A}_j}{\omega'-\Tilde{z}_j} \\
    =
    \sum_{\substack{i,j \\ \Im{z_i}<0 \\ \Im{\Tilde{z}_j}>0 }} \frac{A_i \Tilde{A}_j}{\omega+\Tilde{z}_j-z_i}
    - \sum_{\substack{i,j \\ \Im{z_i}>0 \\ \Im{\Tilde{z}_j}<0 }} \frac{A_i \Tilde{A}_j}{\omega +\Tilde{z}_j-z_i}.
\label{eq:convolutionSOP}
\end{multline}
%
%closing the contour above the real axis. 

\note{
Using the the SOP for $G$, the following integrals can also be computed explicitly: 
\AF{
\begin{eqnarray}
    E_m[G]&=&
    %\lim_{\eta\to0^+}
    \oint_{\Gamma} \frac{dz}{2\pi i} %e^{i\eta\omega}
    e^{i z 0^+}
    z^m G(z)
    \nonumber \\[6pt]
    &=&\sum_{\substack{i \\ \Im{z_i}>0}} A_i z^{m}_i,
    \label{eq:moments}
\end{eqnarray}
%
}
where we refer to the term $E_m[G]$ as the $m$-th (regularized) moment of $G$. $\Gamma$ here is a \AF{closed contour in the upper-half complex plane including the real axis plus the enclosing arc}.
We note that for the $m=0$, $m=1$, and $m=2$ moments, $\Gamma$ can be reduced to the real axis using the $1/\omega$ decay of $G$ \AF{(the symmetry of the integration domain is also invoked for $m=2$ to discart odd terms)}.
We underline that if one uses an $n$-th order Lorentzian basis to represent $G(\omega)$ on SOP, the first $2(n-1)$ regularized moments coincide with the moments of its occupied spectral function $\int_{-\infty}^{\mu} d\omega\, \omega^{2(n-1)} A(\omega)$. This is shown in Appendix~\ref{sec:Moments_and_occupiedM}.
}

%, while the moments of its occupied $A$ diverge. Then, in order to have a meaningful result for these moments, it is necessary first to converge the representation basis for $A$ to delta functions ($\delta_i\to0$), and then to perform the integral for the moments of the occupied $A$. Numerically, this consists in controlling the stability of the value of the real-part of $E_{m>2(n-1)}[G]$ in the limit $\delta_i\to0$, and discarding the imaginary-part.

%\TC{To summarize, the evaluation of the moments of a Green's function represented on SOP using an $n$th-Lorentzian-basis set, with Eq.~\eqref{eq:moments}, is meaningful (i.e. it equates to the moments of its occupied spectral function) when the momentum degree is~$m \le2(n-1)$. For higher order moments it is necessary to converge the $n$th-Lorentzian-basis set to a delta basis. This property is very useful when evaluating frequency integrated quantities, e.g. the total energy with the Galitskii-Migdal expression~\cite{Fetter-Walecka1971book,Martin-Reining-Ceperley2016book} (involving a first-order moment) can be computed directly from a G on SOP transformed from a $2^\text{nd}$-Lorentzian-basis set (or higher).}

%%%%%%%%%%% ABOVE TO BE REINTRODUCED IF NEEDED %%%%%%

%Importantly, for the regular Lorentzians, $n=1$, only the zero-order occupied momentum can be computed analytically with Eq.~\eqref{eq:moments}, {\color{red}the higher moments can be evaluated with a convergence study $\Im{z_i}\to0$ of the poles in the SOP (i.e. converge to a delta basis). } \AFnote{Secondo me questo pezzo non e' chiarissimo... convergence study ? serve tenerlo ?} \TCnote{ok parliamone}\\
%\AFnote{Una cosa che manca, penso sia il perche' ci fermiamo a $2(n-1)$. Diciamo fast decay, ma la relazione non e' esplicitata... forse questo sarebbe utile. Penso si veda abbastanza chiaramente dalla penultima equazione.} \TCnote{sono d'accordo. Secondo me i momenti sopra sono comunque legati alla nota precedente. Quindi discutiamo anche di questo} \\
%\AFnote{Moreover, questo stesso risultato si dovrebbe poter ottenere esplicitamente usando le Eqs.~(\ref{eq:TOHT_nlor_basis_res}-\ref{eq:TOHT_nlor_basis_poles}).} \TCnote{secondo me già così mi sembra sufficentemente esteso e andare bene, pero' vediamo insieme}

%This is definitely improved by $n$-Lorentzians, allowing for the computation of higher order moments, very useful when evaluating, e.g., the total energy via the Galitskii-Migdal expression~\cite{Fetter-Walecka1971book,Martin-Reining-Ceperley2016book}.
% SOLVED
%\AFnote{The above proof could be a good candidate for SuppInfo, if any.} \TCnote{secondo me meglio un'appendice}\AFnote{yess, anche secondo me}

%Importantly, the regular Lorentzians, $n=1$, only the zero-order momentum (the normalization) can be computed without resorting to the exponential regularization factor. 

%\AFnote{Here we could also add a section about "SOP contraction", that is a relevant abstract operation on SOP, if we find out an effective algorithm.}
%\TCnote{punto di discussione}


==> sec_supplemental_material.tex <==
%========================
\section{Convergence studies at several densities of the HEG}
\label{sec:Convergence studies at all densities of the HEG}
%========================
In this section we show the convergence studies at all densities of~\cite{thisPaper}. Following the method presented in Secs.~\ref{sec:method_HEG}, and particularly~\ref{sec:numerical_details}, of~\cite{thisPaper} at $r_s=4$, we study stability and convergence of the correlation (total minus Fock) energy per particle at $r_s$ from $1$ to $10$. In Figs.~\ref{fig:SI_totEnecG0W0rs1},~\ref{fig:SI_totEnecG0W0rs2},~\ref{fig:SI_totEnecG0W0rs3},~\ref{fig:SI_totEnecG0W0rs4},~\ref{fig:SI_totEnecG0W0rs5},~\ref{fig:SI_totEnecG0W0rs6},~\ref{fig:SI_totEnecG0W0rs7},~\ref{fig:SI_totEnecG0W0rs8},~\ref{fig:SI_totEnecG0W0rs9},~\ref{fig:SI_totEnecG0W0rs10} we plot the convergence study at the different densities.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/convFile_gathered_rs_1.png}
    \caption{Correlation energy $E_\mathrm{corr}$ convergence study obtained with the Galitzki-Migdal formula using a Green function from a $G_0W_0$ calculation for the HEG at $r_s=1$. See Fig.~\ref{fig:totEnecG0W0rs4} of~\cite{thisPaper} for further reference.}
    \label{fig:SI_totEnecG0W0rs1}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/convFile_gathered_rs_2.png}
    \caption{Correlation energy $E_\mathrm{corr}$ convergence study obtained with the Galitzki-Migdal formula using a Green function from a $G_0W_0$ calculation for the HEG at $r_s=2$. See Fig.~\ref{fig:SI_totEnecG0W0rs4} of~\cite{thisPaper} for further reference.}
    \label{fig:SI_totEnecG0W0rs2}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/convFile_gathered_rs_3.png}
    \caption{Correlation energy $E_\mathrm{corr}$ convergence study obtained with the Galitzki-Migdal formula using a Green function from a $G_0W_0$ calculation for the HEG at $r_s=3$. See Fig.~\ref{fig:totEnecG0W0rs4} of~\cite{thisPaper} for further reference.}
    \label{fig:SI_totEnecG0W0rs3}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/convFile_gathered_rs_4.png}
    \caption{Correlation energy $E_\mathrm{corr}$ convergence study obtained with the Galitzki-Migdal formula using a Green function from a $G_0W_0$ calculation for the HEG at $r_s=4$. See Fig.~\ref{fig:totEnecG0W0rs4} of~\cite{thisPaper} for further reference.}
    \label{fig:SI_totEnecG0W0rs4}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/convFile_gathered_rs_5.png}
    \caption{Correlation energy $E_\mathrm{corr}$ convergence study obtained with the Galitzki-Migdal formula using a Green function from a $G_0W_0$ calculation for the HEG at $r_s=5$. See Fig.~\ref{fig:totEnecG0W0rs4} of~\cite{thisPaper} for further reference.}
    \label{fig:SI_totEnecG0W0rs5}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/convFile_gathered_rs_6.png}
    \caption{Correlation energy $E_\mathrm{corr}$ convergence study obtained with the Galitzki-Migdal formula using a Green function from a $G_0W_0$ calculation for the HEG at $r_s=6$. See Fig.~\ref{fig:totEnecG0W0rs4} of~\cite{thisPaper} for further reference.}
    \label{fig:SI_totEnecG0W0rs6}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/convFile_gathered_rs_7.png}
    \caption{Correlation energy $E_\mathrm{corr}$ convergence study obtained with the Galitzki-Migdal formula using a Green function from a $G_0W_0$ calculation for the HEG at $r_s=7$. See Fig.~\ref{fig:totEnecG0W0rs4} of~\cite{thisPaper} for further reference.}
    \label{fig:SI_totEnecG0W0rs7}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/convFile_gathered_rs_8.png}
    \caption{Correlation energy $E_\mathrm{corr}$ convergence study obtained with the Galitzki-Migdal formula using a Green function from a $G_0W_0$ calculation for the HEG at $r_s=8$. See Fig.~\ref{fig:totEnecG0W0rs4} of~\cite{thisPaper} for further reference.}
    \label{fig:SI_totEnecG0W0rs8}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/convFile_gathered_rs_9.png}
    \caption{Correlation energy $E_\mathrm{corr}$ convergence study obtained with the Galitzki-Migdal formula using a Green function from a $G_0W_0$ calculation for the HEG at $r_s=9$. See Fig.~\ref{fig:totEnecG0W0rs4} of~\cite{thisPaper} for further reference.}
    \label{fig:SI_totEnecG0W0rs9}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/convFile_gathered_rs_10.png}
    \caption{Correlation energy $E_\mathrm{corr}$ convergence study obtained with the Galitzki-Migdal formula using a Green function from a $G_0W_0$ calculation for the HEG at $r_s=10$. See Fig.~\ref{fig:totEnecG0W0rs4} of~\cite{thisPaper} for further reference.}
    \label{fig:SI_totEnecG0W0rs10}
\end{figure}

==> supplemental_material_aux_manual.tex <==


